Quantum diffusion map for nonlinear dimensionality reduction

Inspired by random walk on graphs, diffusion map (DM) is a class of unsupervised machine learning that offers automatic identification of low-dimensional data structure hidden in a high-dimensional dataset. In recent years, among its many applications, DM has been successfully applied to discover relevant order parameters in many-body systems, enabling automatic classification of quantum phases of matter. However, classical DM algorithm is computationally prohibitive for a large dataset, and any reduction of the time complexity would be desirable. With a quantum computational speedup in mind, we propose a quantum algorithm for DM, termed quantum diffusion map (qDM). Our qDM takes as an input $N$ classical data vectors, performs an eigen-decomposition of the Markov transition matrix in time $O(\log^3 N)$, and classically constructs the diffusion map via the readout (tomography) of the eigenvectors, giving a total expected runtime proportional to $N^2 \text{polylog}\, N$. Lastly, quantum subroutines in qDM for constructing a Markov transition matrix, and for analyzing its spectral properties can also be useful for other random walk-based algorithms.

==> quantikz.tex <==

    \begin{quantikz}
        &&&\lstick{$\ket{0}$}&\gate{R\qty(\frac{1}{\sqrt{d_i}})}&\meter{$\ket{1}$}\\
        \lstick{$\ket{\vb*{0}}$}&\gate{H}\qwbundle[alternate]{}&\ctrlbundle{1}&\gate{\text{QFT}^\dagger}\qwbundle[alternate]{}&\ctrlbundle{-1}&\trash{\text{trash}}\qwbundle[alternate]{}\\
        \lstick{$\ket{+}$}&\qw &\gate[wires=3]{\mathcal{U}_D}&\qw &\qw&\trash{\text{trash}} \\
        \lstick{$\ket{{\mathbbm{1}}}$}&\qwbundle[alternate]{} &\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\rstick{$\hat{D}^{-1}$}\qwbundle[alternate]{}\\
        \lstick{$\ket{\vb*{0}}$}&\qwbundle[alternate]{} &\qwbundle[alternate]{}& \qwbundle[alternate]{}& \qwbundle[alternate]{}&\trash{\text{trash}}\qwbundle[alternate]{} \\
    \end{quantikz}
    
    \begin{quantikz}
        \qwbundle[alternate]{}&\gate[wires=4]{\text{QPE}_D}\qwbundle[alternate]{}&\qwbundle[alternate]{} \\
        \qw&\qw&\qw \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{} \\
        \qw&\qw&\qw
    \end{quantikz}
    
    \begin{quantikz}
        \lstick[wires=2]{$\ket{\vb*{0}}$}\qw&\gate[wires=4]{\text{QPE}_P}&\gate[wires=4]{U_f}\gategroup[4,steps=2,style={dashed,
                   rounded corners,fill=blue!20, inner xsep=2pt},
                   background]{{repeat $O(1)$ steps}}&\gate[wires=4]{U_P}& \meter{}\rstick[wires=2]{$\ket{\widetilde{\frac{\lambda_i}{2}}}$} \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}& \meter{}\qwbundle[alternate]{} \\
        \lstick[wires=2]{$\ket{\psi_0}$}\qw&\qw&\qw&\qw&\meter{$\ket{2}$} \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}\rstick{$\ket{v_i}$}
    \end{quantikz}
    
    \begin{quantikz}
        \qwbundle[alternate]{}&\gate[wires=2]{\text{QPE}_P}\qwbundle[alternate]{}&\qwbundle[alternate]{} \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}
    \end{quantikz}
    
    \begin{quantikz}
        \qwbundle[alternate]{}&\gate{H}\qwbundle[alternate]{}&\ctrlbundle{1}&\gate{\text{QFT}^\dagger}\qwbundle[alternate]{}&\qwbundle[alternate]{} \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\gate{e^{iX_3(P)t}}\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}
    \end{quantikz}
    
    \begin{quantikz}
        \qw&\gate[wires=4]{U_P}\qw&\qw \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{} \\
        \qw&\qw&\qw \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}
    \end{quantikz}
    
    \begin{quantikz}
       \qw&\gate[wires=4]{\rotatebox{0}{$\text{QPE}_P^\dagger$}}\qw&\gate[wires=4]{\rotatebox{0}{$2\dyad{\vb*{0}}\otimes\dyad{\phi_0}-I$}}\qw&\gate[wires=4]{\rotatebox{0}{$\text{QPE}_P$}}\qw&\qw \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{} \\
        \qw&\qw&\qw&\qw&\qw \\
        \qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}
    \end{quantikz}
    
    \begin{quantikz}
        &&&\lstick{$\ket{0}_\text{anc}$}&\gate{R\qty(\frac{1}{\sqrt[4]{d_i}})}&\meter{$\ket{1}$}\\
        \lstick{$\ket{\vb*{0}}_\val$}&\gate{H}\qwbundle[alternate]{}&\ctrlbundle{1}&\gate{\text{QFT}^\dagger}\qwbundle[alternate]{}&\ctrlbundle{-1}&\trash{\text{trash}}\qwbundle[alternate]{}\\
        \lstick{$\ket{+}_R$}&\qw &\gate[wires=3]{\mathcal{U}_D}&\qw &\qw&\trash{\text{trash}} \\
        \lstick{$\ket{{\mathbbm{1}}}_\svec$}&\qwbundle[alternate]{} &\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\rstick{$\hat{D}^{-1/2}$}\qwbundle[alternate]{}\\
        \lstick{$\ket{\vb*{0}}_\J$}&\qwbundle[alternate]{} &\qwbundle[alternate]{}& \qwbundle[alternate]{}& \qwbundle[alternate]{}&\trash{\text{trash}}\qwbundle[alternate]{} \\
    \end{quantikz} 
    
    \begin{quantikz}
        &&&&&\lstick{$\ket{0}_\text{anc}$}&\gate{R\qty(\frac{1}{\sqrt{d_i}})}&\meter{$\ket{1}$}\\
        &&\lstick{$\ket{\vb*{0}}_\text{deg}$}&\gate{H}\qwbundle[alternate]{}&\ctrlbundle{2}&\gate{\text{QFT}^\dagger}\qwbundle[alternate]{}&\ctrlbundle{-1}&\trash{\text{trash}}\qwbundle[alternate]{}\\
        \lstick{$\ket{\vb*{0}}_\val$}&\gate{H}\qwbundle[alternate]{}&\ctrlbundle{1}&\gate{\text{QFT}^\dagger}\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\rstick{$\ket{\widetilde{\lambda_i}}_\val$}\qwbundle[alternate]{}\\
        \lstick{$\ket{+}_R$}&\qw &\gate[wires=2]{e^{iX_3(S)t}}&\qw&\gate[wires=3]{\mathcal{U}_D}&\qw &\qw&\trash{\text{trash}} \\
        \lstick{$\ket{\psi_0}_\svec$}&\qwbundle[alternate]{}&\qwbundle[alternate]{} &\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\rstick{$\ket{v_i}_\svec$}\qwbundle[alternate]{}\\
        &&&\lstick{$\ket{\vb*{0}}_\J$}&\qwbundle[alternate]{}&\qwbundle[alternate]{}&\qwbundle[alternate]{} &\trash{\text{trash}}\qwbundle[alternate]{} \\
    \end{quantikz}    
